Rationality-Robust Information Design: Bayesian Persuasion under Quantal Response

Classic mechanism/information design imposes the assumption that agents are fully rational, meaning each of them always selects the action that maximizes her expected utility. Yet many empirical evidence suggests that human decisions may deviate from this full rationality assumption. In this work, we attempt to relax the full rationality assumption with bounded rationality. Specifically, we formulate the bounded rationality of an agent by adopting the quantal response model (McKelvey and Palfrey, 1995). We develop a theory of rationality-robust information design in the canonical setting of Bayesian persuasion (Kamenica and Gentzkow, 2011) with binary receiver action. We first identify conditions under which the optimal signaling scheme structure for a fully rational receiver remains optimal or approximately optimal for a boundedly rational receiver. In practice, it might be costly for the designer to estimate the degree of the receiver's bounded rationality level. Motivated by this practical consideration, we then study the existence and construction of robust signaling schemes when there is uncertainty about the receiver's bounded rationality level.

==> Paper/abstract.tex <==






Bayesian persuasion in information design 
studies how an information-advantaged sender can 
%incentivize 
influence a receiver to take the sender's preferred action
by designing an information disclosure policy, 
a.k.a., a signaling scheme.
%to take the sender's preferred action. 
Most works in Bayesian persuasion
assume that the receiver is {\em fully rational}, i.e., % if %in the sense that
she always selects the action that 
maximizes her expected utility.
%given her Bayesian posterior belief about the state. 
Yet empirical evidence suggests that human decisions
may deviate from this expected utility theory. 
% Given such background,
In this work, we relax the full rationality assumption and consider a {\em boundedly rational} receiver. In particular,
% relax receiver's full rationality assumption 
we formulate the receiver's boundedly rationality by adopting the classical model of quantal response, which captures the receiver's possible deviation from full rationality through incorporating noises in the receiver's process of utility estimation during decision making.
%which allows the receiver to have random additive error
%while estimating her expected utility induced for each action
%and then select an action that has the highest random utility.
Focusing on a fundamental persuasion model 
with binary action, we seek to understand 
how the receiver's boundedly rational behavior 
impacts the design of {\em optimal} signaling schemes,
% whether the structure of optimal signaling scheme 
% for a fully rational receiver preserve or
% approximately preserve when the receiver becomes boundedly rational, 
and whether there exists {\em robust} signaling scheme when the 
receiver's boundedly rational behavior remains unknown. 
For both questions, we provide positive and negative answers. 
At a high-level, a crucial condition
that governs our answers is whether the sender’s utility depends on the realized state.

For the first question, 
in contrast to the setting with
a fully rational  receiver 
where both {\em censorship} and {\em direct} 
signaling scheme are always optimal \citep{RSV-17},
we show that for a boundedly rational receiver,
the censorship % signaling scheme
remains optimal in {\em state independent sender utility} 
(SISU) environments, but is no longer optimal 
in {\em state dependent sender utility} (SDSU) environments,
and direct signaling scheme is no longer optimal in both environments.
Nonetheless, we show that censorship is
$\Theta(m)$-approximation in SDSU environments, 
and direct signaling scheme is $\Theta(m)$-approximation in both environments, 
where $m$ is the number of states.
% En route, we 
% characterize the optimal signaling scheme 
% in SDSU environments, 
% in which the sender's signal either reveals the true state, 
% or randomizes the receiver's uncertainty on
% only two states.

For the second question, 
we introduce rationality-robust information design
-- a framework in which a signaling scheme 
is designed for a receiver with unknown boundedly rational behavior. 
We show that in SISU environments, 
up to a $2$-approximation factor, 
implementing optimal censorship
signaling scheme of a fully rational receiver is 
rationality-robust for any boundedly rational receiver;
\wtr{but implementing optimal direct
signaling scheme of a fully rational receiver is 
no longer rationality-robust}. 
% a robust signaling scheme that is $2$-approximation for any 
% boundedly rational behavior exists. 
In marked contrast to this positive result, 
in SDSU environments, there exists
no robust signaling scheme that has any bounded approximation.
Nonetheless, for any problem instance with binary state, 
under a reasonable multiplicative boundedness condition
on the receiver's behavior, 
the sender is able to design a signaling scheme whose
approximation ratio depends linearly on the multiplicative error.


 















==> Paper/intro-main-contributions.tex <==
\cj{probably need to wait and see how this subsection reads as a whole after it's done. my first reaction is that maybe we want to have a succinct summary of the main results upfront.}


\paragraph{Bayesian Persuasion under Quantal Response}
We propose a model of bounded rationality based on the 
quantal response in Bayesian persuasion
to study 
rationality-robust information design problems. 
% introduce a framework on Bayesian persuasion under
% quantal response to study 
% rationality-robust information design problems. 
While information design or mechanism design with
bounded rationality under other models 
have been well studied in the literature 
(see \Cref{subsec:related} for a detailed discussions), 
prior to this work, Bayesian persuasion under quantal response
has not been studied before. %in the literature. 

When the receiver is fully rational, 
one can formulate sender's problem on identifying 
optimal signaling schemes as a linear program.
By the revelation principle \citep{KG-11}, 
it is without loss of generality to consider signaling scheme
that has at most $2$ signals.
Hence, optimal signaling scheme can be solved
from the linear program with at most $m$ variables,
where $m$ denotes the number of states. 
% one can formulate the problem on identifying 
% optimal signaling schemes as a linear program 
% with at most $O(m)$ variables,
% where $m$ denotes the number of states. 
When the receiver is boundedly rational, the revelation principle fails.
% for both SISU and SDSU environments with only two signals. 
% the optimal signaling schemes in both SISU and SDSU environments 
% have been well studied and
% admit a 
% share the similar structure -- the optimal signaling schemes  
In \Cref{sec:prelim}, we show that when 
the sender knows receiver's quantal response behavior
(i.e., knows receiver's bounded rationality level $\noiseScale$), 
the problem on identifying an optimal signaling scheme 
can still be formulated as a linear program, denoted by \ref{eq:opt lp},
but with continuous variables and infinite number of constraints.
When the receiver is fully rational, the optimal signaling scheme
in both SISU and SDSU environments admits a simple structure
-- it specifies an order (based on receiver's and sender's utilities)
over all states, and
% uses only $2$ signals where 
one signal is used to 
pool all states below a threshold state, and another signal is 
used to pool all states above a threshold state.
% -- it specifies an order (based on receiver's and sender's utilities)
% over all states, censors all states below a threshold state 
% at a same censorship signal,
% censors all states above a threshold state at another censorship signal,
% and possibly randomizes at the threshold state. 
Relative to a fully rational receiver, a boundedly rational receiver
reacts to the signaling scheme with the same belief updating, 
but taking actions with larger probability 
if the actions are more attractive. 
Therefore one might wonder that whether the optimal signaling scheme for 
a boundedly rational receiver continues to share the similar structure 
(e.g., binary signal space, same state order)
as the one for fully rational receiver.
This turns out to not be the case, as
we provide characterizations on optimal solutions 
to the aforementioned problem \ref{eq:opt lp}
in SISU (see \Cref{sec:state independent}) 
and SDSU (see \Cref{sec:state dependent}) environments. 



% One insight can be obtained from optimal solution characterizations
% is that when the receiver is fully rational,
% the two environments share the similar structure 
% -- a censorship structure --
% on optimal signaling schemes,
% while when the receiver becomes boundedly rational, 
% optimal signaling schemes 
% signaling scheme with censorship structure 
% is no longer optimal for SDSU environments. 

% when the receiver is fully rational, there exists a censorship 
% signaling scheme that is optimal for both SISU and SDSU environments.




\paragraph{Optimality of Censorship Signaling Scheme in SISU Environments}
In \Cref{sec:state independent},
by analyzing 
the dual counterpart, denoted by \ref{eq:opt lp dual}, 
of sender's problem, % optimization problem, 
we show that there exists a signaling scheme that
has {\em censorship} structure that is optimal 
for boundedly rational receiver in SISU environments 
(see \Cref{thm:SISU opt}).
% We establish the optimality % of censorship signaling schemes 
A signaling scheme with censorship structure
(henceforth censorship signaling scheme)
specifies an order over all states, % of the nature,
censors the states below a threshold state together by disclosing 
the same censorship signal for all these states, 
fully reveals the states above the threshold state, 
and partially reveals the threshold state. 
A key observation in our analysis is that every feasible solution
to the dual program \ref{eq:opt lp dual} forms 
a {\em upper convex envelope}
for the function $\Quant$ 
(see \Cref{fig:SISU opt condition} for illustration), 
and we show that there exists a unique upper convex envelope 
(i.e., the optimal censorship signaling scheme) that 
also satisfies the complementary slackness.

Though our characterization shows that 
the optimal censorship signaling scheme
for a boundedly rational receiver in SISU environments
defines the same order 
over the states as the optimal one for a fully rational receiver,
the censorship signaling scheme differs with 
the optimal one for a fully rational receiver 
as the censorship signaling scheme fully reveals 
the states above the threshold state.
Hence, % in SISU environments, 
to achieve optimal persuasion,
% signaling scheme, 
sender generally needs at least $2$ signals, and at most $m$ signals.
% However, unlike the optimal signaling scheme for a fully rational receiver
% which censors all states above the threshold state, 
% the optimal censorship signaling scheme for a bounded rational receiver
% requires the sender to fully reveal 
Moreover, our characterization also deduce 
following insight on the structural property:
The threshold state in
optimal censorship signaling scheme 
is weakly decreasing when the receiver becomes less rational
(see \Cref{prop:SISU threshold state monotonicity}). 
This leads to an insight that in SISU environments, 
the optimal signaling scheme requires the
sender to reveal more information for a less rational receiver.
This structural observation allows us to identify 
a robust signaling scheme when the sender does not have
any knowledge about receiver's bounded rationality in \Cref{sec:robust}.


\paragraph{(Approximately) Optimal Signaling Scheme in SDSU Environments}
Having characterized optimal signaling schemes in SISU environments, 
in \Cref{sec:SDSU optimal}, 
we then proceed to characterize optimal signaling schemes in SDSU environment.
We show that, the optimality of censorship signaling schemes 
is no longer preserved in SDSU environments. 
Instead, we show that (see \Cref{thm:SDSU opt}) there exists an 
optimal signaling scheme in SDSU environments
that has following two properties: 
(i) every signal is used to pool at most two states;
(ii) every pair of states is pooled at most one signal.
Intuitively, property~(i)
says that whenever the receiver sees a signal
from the optimal signaling scheme, 
she can infer that the realized state must 
be one of two particular states. 
From a practical perspective, this property is  
beneficial to a boundedly rational receiver as it 
makes the receiver's state inference relatively easier.
From sender's perspective, 
property~(ii) says that there is no need for the sender to 
pool a pair of states at multiple signals.
These two properties jointly imply that 
$\sfrac{m(m-1)}{2}$ signals suffice to achieve optimal persuasion,
% signaling scheme,
making the implementation of the 
optimal signaling scheme practically feasible.
At a high-level, our characterization for 
optimal signaling scheme in SDSU environments follow
a two-step approach: 
(1) we first show that it is without loss to 
consider signaling schemes that satisfy property (i);
(2) we then take advantage of the property (i) and show that 
it is always best to not pool any pair of states at more than $1$ signal,
we achieve this by decomposing original sender's program
\ref{eq:opt lp} as smaller programs for each pair of states, 
and then use similar previous primal-dual analysis to get the results.

% In practice, there may exist limitations to design 
% a signaling scheme that has $\Omega(m^2)$ signals.\footnote{For example: \wtr{Give motivations here ...}} 
\wt{needs to think about what is the story here?}
Though the optimal signaling scheme in SDSU environments
uses at most $O(m^2)$ signals, it is relative more complex 
than the optimal one for SISU environments. 
In \Cref{sec:SDSU simple approx},
we study approximation upper bounds of signaling schemes 
(e.g., censorship signaling schemes) which admit relatively simpler forms 
(comparing the optimal signaling scheme characterized in \Cref{thm:SDSU opt}).
We show that there exists a signaling
scheme that has the same two properties of the optimal signaling scheme 
but only uses at most $2m$ signals,
and is a $4$-approximation to the optimal signaling scheme. 

% Though censorship signaling schemes are no longer optimal 
% in SDSU environments, we also show that 


\paragraph{Rationality-robust Information Design}
In above discussions, designing optimal signaling schemes
in both SISU and SDSU environments we consider 
is rationality-oriented
-- the sender needs to exactly know 
receiver’s bounded rationality level.
In practice, the sender may not be able to have 
(or require significant cost to learn) such perfect
knowledge.% of a receiver’s bounded rationality level. 
Motivated by this concern, in \Cref{sec:robust},
we introduce rationality-robust 
information design, 
in which a signaling scheme is
designed for a receiver whose bounded rationality 
level is unknown. 
The goal is to identify robust
signaling schemes -- ones with good (multiplicative) rationality-robust approximation to the optimal
signaling scheme that is tailored to possible receiver’s 
bounded rationality level.

In SISU environments, by leveraging the structural property 
we mentioned before, 
% of optimal signaling scheme established in \Cref{prop:SISU threshold state monotonicity}, 
namely, the optimal signaling scheme for a less rational
receiver requires the sender to reveal more information,
we show that the optimal censorship signaling scheme
for a fully rational receiver achieves a $2$ 
rationality-robust approximation when the sender 
has no knowledge of the receiver's bounded rationality level 
(see \Cref{thm:2 robust approx SISU upperbound}).
We also provide an
example to show the tightness of the result 
(see \Cref{prop:2 robust approx SISU lower bound}).
This suggests that, up to a two factor, 
the knowledge of the receiver's bounded rationality level are
unimportant in SISU environments, 
as the optimal censorship signaling scheme of a fully rational
receiver continues to perform well
no matter how less rational the receiver is. 

In contrast, in SDSU environments, 
we show that there exists no signaling
scheme with bounded rationality-robust approximation ratio, 
when the sender has no knowledge of the receiver’s bounded rationality level
(see \Cref{thm:imposs robust approx SDSU}), 
and this result holds even if the state space is binary.
To show this impossibility result, we construct 
a binary-state problem instance and 
a set of carefully chosen possible bounded rationality levels. 
The key to our approach is by introducing a 
factor-revealing program to lower bound the optimal 
rationality-robust approximation ratio, which we shows that 
the lower bound of the optimal objective value can go to infinite.
This impossibility result indicates that there 
exists a tradeoff between the knowledge of the receiver's rationality level and
the achievable rationality-robustness. 
While it appears challenging to obtain a bounded-factor 
rationality-robust approximation for arbitrary set of rationality levels,
we obtain a simple approximation under a 
boundedness condition on the receiver's rationality level.
In particularly, 
we show that such positive result is possible when the state space is binary
under a certain multiplicative boundedness condition 
(i.e., learning the receiver’s bounded rationality level up to
a multiplicative error) 
on the receiver's bounded rationality levels,
the sender is able to design a signaling scheme
whose rationality-robust approximation ratio 
depends linearly on the multiplicative error 
(see \Cref{thm:SDSU binary robust}). 

\input{Paper/intro-table}



% ============== Below is Yiding's Sketch ==================

% Introduce SISU and SDSU. Two environments are similar 
% under fully rationality. Describe optimal policy under rationality, introduce censorship signaling scheme.


% SISU discussion. Optimality of censorship signaling scheme.
% Monotonicity of threshold state. Technique: 
% Optimal policy can be formulated as LP.  
% Primal dual analysis.

% SDSU discussion. Censorship/monotone partition is no longer optimal,
% at most $m$ approximation. 
% Optimal signaling scheme characterization. 
% 4-approximation signaling scheme.

% Introduce rationality-robustness robustness.

% SISU robust result.

% SDSU robust result. Also mention the tradeoff between
% knowledge of rationality and robustness.

% ============== Above is Yiding's Sketch ==================



==> Paper/intro-table.tex <==









\begin{table}[h!]
\fontsize{10}{18}\selectfont
\centering
%\caption{Approximation ratios of 
%(approximate) optimal signaling schemes}
\caption{Approximation ratio upper bounds for signaling schemes with constraints on the number of signals.}
\label{tabel:summary number of signal}
\vspace{8pt}
\begin{tabular}{c|ccc|}
\cline{2-4}
                                        & \multicolumn{1}{c|}{Fully Rational}     & \multicolumn{2}{c|}{Boundedly Rational}               \\ \hline
\multicolumn{1}{|c|}{Number of signals} & \multicolumn{1}{c|}{SISU/SDSU}          & \multicolumn{1}{c|}{\ \  SISU \ \  }        & SDSU    \\ \hline
\multicolumn{1}{|c|}{2}                 & % \multicolumn{1}{C{.17\textwidth}|}{$1^{(\dagger)}$ \par previous work} 
\multicolumn{1}{c|}{
$\begin{array}{cc}
     1^{~(\dagger)} \\[-6pt]
     {\scriptsize \text{[e.g., \cite{RSV-17}]}} 
\end{array}$
} 
& \multicolumn{2}{c|}{
$\begin{array}{cc}
     4m^{~(\dagger)(\ddagger)} \\[-6pt]
     {\scriptsize \text{[\Cref{prop: SDSU censorship approx LB}]}}
\end{array}$
}       \\ \hline
\multicolumn{1}{|c|}{$O(m)$}            
& \multicolumn{1}{c|}{
$\begin{array}{cc}
     1^{~(*)} \\[-6pt]
     {\scriptsize \text{[e.g., \cite{RSV-17}]}}
\end{array}$
}          
& \multicolumn{1}{c|}{
$\begin{array}{cc}
     1^{~(*)} \\[-6pt]
     {\scriptsize \text{[\Cref{thm:SISU opt}]}}
\end{array}$
}              & 
$\begin{array}{cc}
     4 \\[-6pt]
     {\scriptsize \text{[\Cref{thm:SDSU 4 approx}]}}
\end{array}$
\\ \hline
\multicolumn{1}{|c|}{$O(m^2)$}          
& \multicolumn{3}{c|}{
$\begin{array}{cc}
     1 \\[-6pt]
     {\scriptsize \text{[\Cref{thm:SDSU opt}]}}
\end{array}$}                                                                        \\ \hline
\end{tabular}

\fontsize{9}{13}\selectfont
\vspace{8pt}
{
$^{(\dagger)}$ achieved by censorship signaling scheme with 
additionally pooling for states above the threshold state; \\
$^{(\ddagger)}$ approximation is tight in order for SDSU environments;
$^{(*)}$ achieved by censorship signaling scheme.
}
\end{table}





==> Paper/state-dependent-opt.tex <==
\newcommand{\optsignalspace}{\signalspace^*}
\newcommand{\ked}{^{(k)}}
\newcommand{\instance}{\mathcal{I}}
\newcommand{\oneed}{^{(1)}}
\newcommand{\twoed}{^{(2)}}
\newcommand{\aggregateprob}{p_{ij}}
\newcommand{\aggregateproba}{\aggregateprob\oneed}
\newcommand{\aggregateprobb}{\aggregateprob\twoed}

\newcommand{\optschemeSISUnew}{\signalscheme^*}
\newcommand{\optsignalspaceSISUnew}{\widetilde{\signalspace}^*}
\newcommand{\optschemeSISUcensor}{\widetilde{\signalscheme}^*}

In this subsection, we provide a characterization 
of the optimal signaling schemes.
Unlike SDSU environments for 
a fully rational receiver (\Cref{lem:opt fully rational})
or SISU environments for a boundedly rational receiver
(\Cref{thm:opt state independent})
where the optimal signaling scheme is a censorship signaling scheme,
the optimal signaling scheme for a boundedly rational receiver 
in SDSU environments may not be a censorship signaling scheme.
In fact, the optimal censorship signaling scheme
is an $\Omega(m)$ approximation to the optimal signaling schemes
(see \Cref{thm:monotone partition lower bound}).
Nonetheless, the optimal signaling scheme still admits 
the following structure.
This structure as well as the technical lemmas in its proof
are also used to establish the 
approximation/robustness guarantee of signaling schemes
in the later parts of the paper (\Cref{sec:SDSU simple approx},
\Cref{sec:SDSU simple approx lower bound}
and \Cref{sec:robust}).

\begin{theorem}
\label{thm:SDSU opt}
In SDSU environments, for a boundedly rational receiver,
there exists an optimal signaling scheme $\optscheme$
whose signal space $\optsignalspace$
has at most $\frac{m(m+1)}{2}$ signals.
More specifically,
the optimal signaling scheme $\optscheme$
satisfies the following two properties:
\begin{enumerate}
    \item[(i)] each signal $\signal\in\optsignalspace$
is induced by at most two states,
i.e., $|\supp(\posterior(\signal))|\leq 2$;
    \item[(ii)] each pair of states $(i, j)$
is pooled at most one signal,
i.e., $|\{\signal\in \optsignalspace:
\supp(\posterior(\signal)) = \{i,j\}\}| \leq 1$.
\end{enumerate}
\end{theorem}

\begin{remark}
The above theorem says that it is possible to achieve optimal signaling scheme using $O(m^2)$ signals.
As we further show in \Cref{sec:SDSU simple approx},
there exists a 4-approximated signaling scheme with 
at most $2m$ signals,
and an $4m$-approximated signaling scheme with binary signals.
It remains as an open question whether 
the optimal signaling scheme requires $\Omega(m^2)$ signals.
% \cj{hmm, this remark might need a bit more context.}
\end{remark}




We now provide intuitions of the two properties of the optimal signal scheme characterized in the above theorem.
%Intuitively, 
%For the optimal signaling scheme in \Cref{thm:SDSU opt},
Property~(i)
says that whenever the receiver sees a signal
from the optimal signaling scheme, 
she can infer that the realized state must 
be one of two particular states. 
From a practical perspective, this property is  
beneficial to a boundedly rational receiver as it 
makes the receiver's state inference easier.
From the sender's perspective, 
property~(ii) says that, 
for any pair of states, the sender only needs to design at most one pooling signal.
%there is no need for the sender to 
%pool a pair of states at multiple pooling signals. 
% Together with property~(ii),
The size of the signal space, that is weakly smaller than
$\sfrac{m(m+1)}{2}$, immediately follows from these two properties:
\cjr{there are at most $\sfrac{m(m-1)}{2}$ signals that are induced by pairs of states and $m$ signals induced by single states.}
%this constraint.
%then immediately 
%follows from that there are at most $\sfrac{m(m+1)}{2}$ pairs of states.

Note that since SISU environment is a special case of SDSU environment (with sender utility
$\senderU_i = 1, \forall i\in[m]$), \Cref{thm:SISU opt} and \Cref{thm:SDSU opt} provide two different characterizations of signaling schemes that 
both are optimal for SISU environments.
For a SISU environment,
let $\optschemeSISUcensor$ (resp. $\optschemeSISUnew$) 
be the optimal signaling scheme characterized in 
\Cref{thm:SISU opt} (resp. \Cref{thm:SDSU opt}) 
Below we show that how to use optimal censorship signaling scheme
$\optschemeSISUcensor$ to construct signaling scheme
$\optschemeSISUnew$ that is also optimal (see \Cref{ex: comparison}
for illustration).
% (the validity of the construction is proved in \Cref{lem:SDSU opt step 1}).
% the two optimal signaling schemes and illustrate their similarities and differences (see \Cref{ex: comparison} for a graphical comparison).
% (i.e., a censorship signaling scheme) 
% and $\optschemeSISUnew$ be the optimal signaling scheme 
% characterized in \Cref{thm:SDSU opt}.
%In \Cref{thm:SISU opt}, we show that in SISU environments, 
%there exists a censorship signaling scheme that is optimal.
%Since SISU environments is a special case of SDSU environments (with sender utility
%$\senderU_i = 1, \forall i\in[m]$), 
%\Cref{thm:SDSU opt} provides an alternative optimal signaling scheme for SISU environments.
%Below we compare the two optimal schemes and illustrate their similarities and differences (see \Cref{ex: %comparison} for a comparison).
%Consider an SISU environment,
Fix the same permutation over the state space $[m]$ of signaling scheme 
$\optschemeSISUcensor$.
Let the pooling signal be 
$\censorshipsignal \in [\receiverU_{k}, \receiverU_{k+1}]$
for some state $k\in[\censorshipstate]$.
Signaling scheme $\optschemeSISUnew$ only differs from 
%the signaling scheme 
$\optschemeSISUcensor$
on the states below the threshold state.
\Cref{lem:SDSU opt step 1} shows that 
there exists a set of signals $\{\signal\}$
such that each signal $\signal$ 
satisfies $\supp(\posterior(\signal)) = \{i, j\}$
where $i \le k$, $j \in [k+1, \censorshipstate]$,
and $\expect[i \sim \posterior(\signal)]{\receiverU_i} = \censorshipsignal$.
% As we demonstrate later (see the proof of \Cref{lem:SDSU opt step 1}),
% this way to decouple pooling a set of states in $\optschemeSISUcensor$  to 
% pooing pairs of states in $\optschemeSISUnew$
% is feasible and $\optschemeSISUnew$ indeed achieves
% the same expected sender utility as the signaling scheme $\optschemeSISUcensor$.
% \cj{this last sentence is a bit hard to parse.}
%there indeed exists
%an optimal signaling scheme $\optschemeSISUnew$ 
%in SISU environments that captures
%the above two properties 
%(see \Cref{ex: comparison} for a comparison):

\begin{figure}[H]
\centering
%
%
% \subfloat[
% \label{ex: opt binary censor}
% Optimal signaling scheme defined in
% \Cref{thm:SDSU opt}.
% ]{
% \input{plots/figure-SDSU-opt-five-state-a}
% }~
%
%
\subfloat[
\label{ex: opt censor}
% ss.
]{
\input{plots/figure-SDSU-opt-five-state-b}
}\qquad\qquad
%
%
\subfloat[
\label{ex: opt binary censor}
% Optimal censorship signaling scheme defined in
% \Cref{thm:SISU opt}.
]{
\input{plots/figure-SDSU-opt-five-state-c}
}
\caption{\label{ex: comparison}
Graphical illustration for the structure of
optimal signaling schemes characterized in \Cref{thm:SISU opt} (\Cref{ex: opt censor}) and \Cref{thm:SDSU opt} (\Cref{ex: opt binary censor})
in a SISU environment.
Each state is the black dot, and all the states in a gray shaded region
imply that there exists a signal induced from 
these states. % they are pooled together.
In both figures, 
the receiver is fully rational, i.e., $\noiseScale = \infty$.
The SISU environment is specified as below:
$\receiverU_1 = -1.5, \receiverU_2 = 0.5,
\receiverU_3 = 1, \receiverU_4 = 1.5,
\receiverU_5 = 2$, 
and $\senderU_i = 1, \prior_i =  0.2, \forall i \in[5]$.
For this problem instance, it can be shown that
a censorship signaling scheme $\optschemeSISUcensor$  
(\Cref{ex: opt censor}) 
is optimal: $\optsignalspaceSISUnew = \{\signal_1, \signal_2, \signal_3\}$ , 
$\optschemeSISUcensor_i(\signal_1)=1, \forall i\in[3];
\optschemeSISUcensor_4(\signal_2) = 1;
\optschemeSISUcensor_5(\signal_3) = 1$.
Meanwhile, 
a signaling scheme $\optscheme$ (\Cref{ex: opt binary censor}) 
that satisfies the two properties in \Cref{thm:SDSU opt}
is also optimal:
$\optsignalspace = \{\signal_1, \signal_2, \signal_3, \signal_4\}$,
$\optscheme_1(\signal_1) = \sfrac{1}{3}, 
\optscheme_2(\signal_1) = 1;
\optscheme_1(\signal_2) = \sfrac{2}{3}, 
\optscheme_3(\signal_2) = 1;
\optscheme_4(\signal_3) = 1;
\optscheme_5(\signal_4) = 1.$
% \cj{might make sense to explain what represents state and signals in the figure}
}
\end{figure}




\paragraph{Proof overview of \Cref{thm:SDSU opt}.}
At a high level, the proof of \Cref{thm:SDSU opt}
proceeds in two steps.
First, we present a reduction from arbitrary signaling schemes 
to signaling schemes that satisfy property (i).
Specifically,
given an arbitrary signaling scheme $\signalscheme$,
we can construct a new signaling scheme $\signalscheme\primed$
which satisfies property~(i) and 
achieves the same expected sender utility 
as the original signaling scheme.\footnote{In the remaining of 
this subsection,
we use superscript $\dagger$
to denote the constructed signaling schemes
satisfying property~(i),
and superscript $\ddagger$
to denote the constructed signaling schemes
satisfying properties~(i) (ii).}
In the second step, we provide an approach 
to convert any signaling scheme $\signalscheme\primed$ 
which satisfies property~(i)
to a new signaling scheme $\signalscheme\doubleprimed$ 
which satisfies both properties (i) (ii),
and achieves weakly higher expected sender utility.
% In particular, 
Informally,
given a signaling scheme $\signalscheme\primed$
from the first step, 
we can % try to 
obtain the
% our desired 
signaling scheme 
$\signalscheme\doubleprimed$ by 
optimizing the pooling structure 
for each pair of states while holding signals from 
all other pairs fixed. 
Loosely speaking, this reduces our task
to identify optimal signaling scheme when the
state space is binary.
Hence, we introduce
a technical lemma 
(\Cref{lem:SDSU binary opt}),
showing that the optimal signaling schemes
are censorship signaling schemes when 
the sate space is binary,
which may be of independent interest.

Below we provide detailed discussion and related lemmas for the above mentioned two steps. 
In the end of this subsection, we combine all pieces together to conclude the proof of \Cref{thm:SDSU opt}.

\paragraph{Step 1- reduction to signaling schemes with property~(i).}
In this step, we argue that it is without loss of generality to 
consider signaling schemes that satisfy property~(i) 
in \Cref{thm:SDSU opt}.
\begin{lemma}
\label{lem:SDSU opt step 1}
In SDSU environments, for a boundedly rational receiver,
for an arbitrary signaling scheme~$\signalscheme$,
there exists a signaling scheme $\signalscheme\primed$
with signal space $\signalspace\primed$
such that 
\begin{itemize}[label={-}]
\item each signal $\sigma\in\signalspace\primed$
is induced by at most two states,
\item signaling scheme $\signalscheme\primed$ 
achieves the same expected sender utility
as signaling scheme $\signalscheme$.
\end{itemize}
\end{lemma}

Informally, 
we can construct 
the signaling scheme $\signalscheme\primed$
in \Cref{lem:SDSU opt step 1} as follows.
For each signal $\signal$
in the original signaling scheme $\signalscheme$,
we decompose it into multiple signals, each of which 
is induced by at most two states,
and satisfies some other requirements.
The feasibility of this decomposition is guaranteed
by the following lemma.

\begin{lemma}[\citealp{FTX-22}]
\label{lem:multi label signal to binary label signal random variable}
Let $X$ be a random variable 
with discrete support 
% $\support$.
$\supp(X)$.
There exists a 
positive integer $K$,
a finite set of $K$
random variables $\{X_k\}_{k\in[K]}$,
and 
convex combination coefficients
$\convexcombinbf\in [0, 1]^K$ 
with $\sum_{k\in[K]} \convexcombin_k = 1$
% which satisfy:
such that:
\begin{enumerate}
    \item[(i)] \underline{Bayesian-plausibility}: for each $k\in [K]$, $\expect{X_k} = \expect{X}$;
    \item[(ii)] \underline{Binary-support}:
    for each $k\in[K]$, the size of $X_k$'s support is at most 2,
    i.e., $|\supp(X_k)| \leq 2$
    \item[(iii)] \underline{Consistency}:
    for each $x\in \supp(X)$, 
$\prob{X=x} = \sum_{k\in[K]}
\convexcombin_k\cdot 
\prob{X_k = x}$
\end{enumerate}
\end{lemma}

\begin{proof}[Proof of \Cref{lem:SDSU opt step 1}]
Fix an arbitrary signaling scheme $\signalscheme$
with signal space $\signalspace$.
Recall that $\signalscheme_i(\signal)$
is the probability mass (or density) that signal $\signal$
is realized when the realized state is state $i$.

Now we describe the construction of $\signalscheme\primed$
and its signal space $\signalspace\primed$.
Initially, we set $\signalspace\primed \gets \emptyset$.
For each signal $\signal\in \signalspace$, 
let $\posterior_i(\signal) \triangleq
\frac{\prior_i \signalscheme_i(\signal)}
{\sum_{j\in[m]}\prior_j\signalscheme_j(\signal)}$
be its induced posterior belief for each state $i$.
Consider the following random variable $X$
where 
$\prob{X = \receiverU_i} = \posterior_i(\signal)$
for each $i\in[m]$.
Let integer $K$,
random variables $\{X_k\}_{k\in[K]}$,
and 
convex combination coefficients
$\convexcombinbf\in [0, 1]^K$ 
be the elements in \Cref{lem:multi label signal to binary label signal random variable} for the aforementioned random variable $X$. 
Add $K$ signals $\{\signal^{(1)}, \dots, \signal^{(K)}\}$
into the signal space $\signalspace\primed$,
i.e., 
$\signalspace\primed \gets 
\signalspace\primed \cup \{\signal^{(1)}, \dots, \signal^{(K)}\}$.
For each $k\in[K]$,
set $\signalscheme\primed_i(\signal\ked)
\gets 
\frac{1}{\prior_i}
{\convexcombin_k\cdot \prob{X_k = \receiverU_i}\cdot 
{(\sum_{j\in[m]} \prior_j\signalscheme_j(\signal))}}
$.
Note that this construction ensures that 
\begin{align*}
     \sum_{k\in[K]}
\signalscheme\primed_i(\signal\ked)
&=
\sum_{k\in[K]}
\frac{1}{\prior_i}
{\convexcombin_k\cdot \prob{X_k = \receiverU_i}\cdot 
{\left(\sum_{j\in[m]} \prior_j\signalscheme_j(\signal)\right)}}
% \\
% &
\overset{(a)}{=}
\frac{1}{\prior_i}
\prob{X = \receiverU_i}\cdot 
{\left(\sum_{j\in[m]} \prior_j\signalscheme_j(\signal)\right)}
= \signalscheme_i(\signal)
\end{align*}
where equality~(a) holds due to the ``consistency'' property 
in \Cref{lem:multi label signal to binary label signal random variable}.
Hence, the constructed signaling scheme $\signalscheme\primed$
is feasible.

Additionally, the ``binary-support'' property in \Cref{lem:multi label signal to binary label signal random variable}
ensures that signaling scheme $\signalscheme\primed$ satisfies 
that each signal from $\signalspace\primed$
is induced by at most two states.

Finally, to see 
that signaling scheme $\signalscheme\primed$
achieves the same expected sender utility as signaling scheme $\signalscheme$,
consider the following coupling between these two signaling schemes:
whenever signal $\signal\in \signalspace$
is realized in signaling scheme $\signalscheme$,
sample
the corresponding signal $\signal\ked$ with probability $\convexcombin_k$
for each $k\in[K]$.
This coupling is well-defined due to the
``consistency'' property in 
\Cref{lem:multi label signal to binary label signal random variable}.
Invoking the ``Bayesian-plausibility'' property
in
\Cref{lem:multi label signal to binary label signal random variable},
from the receiver's perspective, 
her expected utility given the posterior belief 
$\posterior(\signal\ked)$
under signaling scheme $\signalscheme\primed$
is the same as 
her expected utility given the posterior belief 
$\posterior(\signal)$ 
under signaling scheme $\signalscheme$.
Thus the probabilities that the receiver takes 
action 1 
are the same in both signaling schemes,
yielding the same expected utility to the sender.
\end{proof}

\paragraph{Step 2- reduction to signaling schemes with properties~(i) and (ii).}
In this step, we argue that it is without loss of generality to 
consider signaling schemes which satisfy properties~(i) and (ii) 
in \Cref{thm:SDSU opt}.

\begin{lemma}
\label{lem:SDSU opt step 2}
In SDSU environments, for a boundedly rational receiver,
given any signaling scheme~$\signalscheme\primed$
with signal space $\signalspace\primed$
where each signal $\sigma\in\signalspace\primed$
is induced by at most two states,
there exists a signaling scheme $\signalscheme\doubleprimed$
with signal space $\signalspace\doubleprimed$
such that 
\begin{itemize}[label={-}]
\item each signal $\sigma\in\signalspace\doubleprimed$
is induced by at most two states,
\item each pair of states is pooled at most one signal,
\item signaling scheme $\signalscheme\doubleprimed$ 
achieves weakly higher expected sender utility
as signaling scheme $\signalscheme\primed$.
\end{itemize}
\end{lemma}

\begin{proof}
Fix an arbitrary signaling scheme
$\signalscheme\primed$
with signal space $\signalspace\primed$
where each signal 
is induced by at most two states.
Below we describe the construction of $\signalscheme\doubleprimed$
and its signal space $\signalspace\doubleprimed$.
Initially, we set $\signalspace\doubleprimed \gets \emptyset$.

For each pair of states $(i, j)$,
let $\signalspace_{ij}\primed \subseteq \signalspace\primed$
be the subset of signals, each of which is induced by state $i$ 
and state $j$,
i.e., $\signalspace_{ij}\primed \triangleq
\{\signal\in \signalspace\primed:\supp(\posterior(\signal)) = 
\{i, j\}\}$.
For ease of presentation,
we introduce auxiliary notations
$\aggregateproba$
(resp.\ 
$\aggregateprobb$)
to denote 
the probability that 
the realized state is $i$
(resp.\ $j$),
and the realized signal is 
from $\signalspace\primed_{ij}$,
i.e., 
$\aggregateproba\triangleq
\int_{\signal\in\signalspace_{ij}\primed}
\prior_i\signalscheme\primed_i(\signal)\,d\signal$
and 
$\aggregateprobb\triangleq
\int_{\signal\in\signalspace_{ij}\primed}
\prior_j\signalscheme\primed_j(\signal)\,d\signal$.
Consider the program~\ref{eq:opt lp}
on the following binary-state instance $\instance_{ij}=
(\hat m, 
\{\hat \prior_k\},
\{\hat \receiverU_k\},
\{\hat \senderU_k\})$:
\begin{align*}
    \hat m \gets 2,\qquad
    \hat \receiverU_1 &\gets \receiverU_i,\qquad
    \hat \receiverU_2 \gets \receiverU_j,\qquad
    \hat \senderU_1 \gets \senderU_i,\qquad
    \hat \senderU_2 \gets \senderU_j,
    \\
    % \hat\noiseScale \gets \noiseScale,\qquad
    &\hat\prior_1\gets
    \frac{\aggregateproba}
    {\aggregateproba+\aggregateprobb},
    \qquad
    \hat\prior_2 \gets
    \frac{\aggregateproba}
    {\aggregateproba+\aggregateprobb}
    %  \hat \prior_1 \gets 
    % \frac{
    % \displaystyle\int_{\signal\in \signalspace_{ij}\primed}
    % \prior_i\signalscheme\primed_i(\signal)\,d\signal
    % }
    % {
    % \displaystyle\int_{\signal\in \signalspace_{ij}\primed}
    % \prior_i\signalscheme\primed_i(\signal)
    % +
    % \prior_j\signalscheme\primed_j(\signal)\,d\signal
    % },
    % \qquad
    % \hat \prior_2 &\gets 
    % \frac{
    % \displaystyle\int_{\signal\in \signalspace_{ij}\primed}
    % \prior_j\signalscheme\primed_j(\signal)\,d\signal
    % }
    % {
    % \displaystyle\int_{\signal\in \signalspace_{ij}\primed}
    % \prior_i\signalscheme\primed_i(\signal)
    % +
    % \prior_j\signalscheme\primed_j(\signal)\,d\signal
    % }
\end{align*}
Notably, 
% after dividing $\{\signalscheme\primed_i(\signal),
% \signalscheme\primed_j(\signal)\}$
% by 
% $
% % \left(
% \int_{\signal\in \signalspace_{ij}\primed}
%     \prior_j\signalscheme\primed_j(\signal)+
%     \prior_j\signalscheme\primed_j(\signal)\,d\signal
%     % \right)
    % $,
% we obtain 
$\left\{
\frac{\prior_i\signalscheme\primed_i(\signal)}{
% \int_{\signal\in\signalspace_{ij}\primed}
% \prior_i\signalscheme\primed_i(\signal)\,d\signal
\aggregateproba
}
\cdot 
\indicator{\signal\in \signalspace_{ij}\primed},
\frac{\prior_j\signalscheme\primed_j(\signal)
}{
% \int_{\signal\in\signalspace_{ij}\primed}
% \prior_j\signalscheme\primed_j(\signal)\,d\signal
\aggregateprobb
}
\cdot \indicator{\signal\in \signalspace_{ij}\primed}
\right\}$
is a feasible solution 
of program~\ref{eq:opt lp}
on the binary-state instance $\instance_{ij}$.
Now, let 
$\{\hat\signalscheme^*_1(\signal),\hat\signalscheme^*_2(\signal)\}$
with signal space $\hat\signalspace_{ij}^*$
be the optimal solution of program~\ref{eq:opt lp}
on the binary-state instance $\instance_{ij}$.
We add signals from $\hat\signalspace_{ij}^*$
into the signal space $\signalspace\doubleprimed$,
i.e., $\signalspace\doubleprimed\gets \signalspace\doubleprimed
\cup \hat\signalspace_{ij}^*$,
and
set $\signalscheme\doubleprimed_i(\signal) \gets 
\frac{\aggregateproba}{\prior_i}
    \cdot
    \hat\signalscheme_1^*(\signal)$,
    $\signalscheme\doubleprimed_j(\signal) \gets 
% \left(\int_{\signal'\in \signalspace_{ij}\primed}
%     \prior_j\signalscheme\primed_j(\signal')+
%     \prior_j\signalscheme\primed_j(\signal')\,d\signal'
%     \right)
%     \cdot
\frac{\aggregateprobb}{\prior_j}\cdot 
    \hat\signalscheme_2^*(\signal)$
    for each signal $\signal \in \hat\signalspace_{ij}^*$.
It is straightforward
to verify that the constructed signaling scheme 
$\signalscheme\doubleprimed$ 
with signal space $\signalspace\doubleprimed$
is feasible, and 
each signal $\signal\in\signalspace\primed$
is induced by at most two states by construction.

Now we argue that 
each pair of states in signaling scheme $\signalscheme\doubleprimed$
is pooled at most one signal.
By our construction of 
signaling scheme $\signalscheme\doubleprimed$,
it is sufficient to show
that for each pair of states $(i, j)$,
the optimal solution 
$\{\hat \signalscheme_i^*(\signal),
\hat \signalscheme_j^*(\signal)\}$
in program~\ref{eq:opt lp}
on binary-state instance $\instance_{ij}$
is a censorship signaling scheme (and thus
it is pooled at most one signal).
We prove this statement by leveraging 
the following lemma (\Cref{lem:SDSU binary opt})
that characterizes the optimal 
signaling scheme of any binary state instance 
is indeed a censorship signaling scheme. 
The proof, deferred to \Cref{apx:SDSU proof},
is based on a primal-dual 
analysis similar to the one for \Cref{thm:opt state independent}.
\begin{lemma}
\label{lem:SDSU binary opt}
In SDSU environments with binary state space (i.e., $m=2$),
there exists a censorship signaling scheme
that is an optimal signaling scheme.
\end{lemma}
Finally, we verify that expected sender utility $\Payoff{\signalscheme\doubleprimed}$
is weakly higher than 
the expected sender utility $\Payoff{\signalscheme\primed}$.
Note that 
\begin{align*}
    \Payoff{\signalscheme\primed} 
    &\overset{(a)}{=}
    \sum_{(i,j)}
    \displaystyle\int_{\signal \in \signalspace_{ij}\primed}
    \left(\prior_i\senderU_i\signalscheme\primed_i(\signal)
    +
    \prior_j\senderU_j\signalscheme\primed_j(\signal)
    \right)
    \Quant(\signal)
    \,d\signal
    \\
    &=
    \sum_{(i,j)}
    \left(
    \aggregateproba + \aggregateprobb
    \right)
    \displaystyle\int_{\signal \in \signalspace_{ij}\primed}
    \left(
    \frac{\aggregateproba}
    {\aggregateproba+\aggregateprobb}
    \senderU_i
    \frac{\prior_i\signalscheme\primed_i(\signal)}
    {\aggregateproba}
    +
    \frac{\aggregateprobb}
    {\aggregateproba+\aggregateprobb}
    \senderU_i
    \frac{\prior_j\signalscheme\primed_i(\signal)}
    {\aggregateprobb}
    \right)
    \Quant(\signal)
    \,d\signal
    \\
    &\overset{(b)}{\leq}
    \sum_{(i,j)}
    \left(
    \aggregateproba + \aggregateprobb
    \right)
    \displaystyle\int_{\signal \in \signalspace_{ij}\primed}
    \left(
    \frac{\aggregateproba}
    {\aggregateproba+\aggregateprobb}
    \senderU_i
    \frac{\prior_i\signalscheme\doubleprimed_i(\signal)}
    {\aggregateproba}
    +
    \frac{\aggregateprobb}
    {\aggregateproba+\aggregateprobb}
    \senderU_i
    \frac{\prior_j\signalscheme\doubleprimed_i(\signal)}
    {\aggregateprobb}
    \right)
    \Quant(\signal)
    \,d\signal
    \\
    &\overset{}{=}
    \sum_{(i,j)}
    \displaystyle\int_{\signal \in \signalspace_{ij}\primed}
    \left(\prior_i\senderU_i\signalscheme\doubleprimed_i(\signal)
    +
    \prior_j\senderU_j\signalscheme\doubleprimed_j(\signal)
    \right)
    \Quant(\signal)
    \,d\signal
    \\
    &\overset{(c)}{=}
    \Payoff{\signalscheme\doubleprimed} 
\end{align*}
where equalities~(a) (c) use \Cref{prop:opt lp}.
To see why inequality~(b) holds,
note that the left-hand side of 
inequality~(b) is the objective value 
of solution 
$\left\{
\frac{\prior_i\signalscheme\primed_i(\signal)}{
% \int_{\signal\in\signalspace_{ij}\primed}
% \prior_i\signalscheme\primed_i(\signal)\,d\signal
\aggregateproba
}
\cdot 
\indicator{\signal\in \signalspace_{ij}\primed},
\frac{\prior_j\signalscheme\primed_j(\signal)
}{
% \int_{\signal\in\signalspace_{ij}\primed}
% \prior_j\signalscheme\primed_j(\signal)\,d\signal
\aggregateprobb
}
\cdot \indicator{\signal\in \signalspace_{ij}\primed}
\right\}$
in program~\ref{eq:opt lp}
on binary-state instance $\instance_{ij}$,
while the right-hand side of inequality~(b),
by the construction of $\signalscheme\doubleprimed$,
is the optimal objective value in this program.
\end{proof}



Now we are ready to prove \Cref{thm:SDSU opt}.
\begin{proof}[Proof of \Cref{thm:SDSU opt}]
Invoking \Cref{lem:SDSU opt step 1}
and \Cref{lem:SDSU opt step 2},
we know that 
there exists an optimal signaling scheme 
where 
(i) each signal is induced by at most two states,
and 
(ii) each pair of states pools on at most one signal.
Note that property~(i) and property~(ii) together 
imply that its signal space has $\frac{m(m+1)}{2}$ signals.
\end{proof}



